Fashion Captioning: Towards Generating Accurate Descriptions with Semantic Rewards

Generating accurate descriptions for online fashion items is important not only for enhancing customers' shopping experiences, but also for the increase of online sales. Besides the need of correctly presenting the attributes of items, the expressions in an enchanting style could better attract customer interests. The goal of this work is to develop a novel learning framework for accurate and expressive fashion captioning. Different from popular work on image captioning, it is hard to identify and describe the rich attributes of fashion items. We seed the description of an item by first identifying its attributes, and introduce attribute-level semantic (ALS) reward and sentence-level semantic (SLS) reward as metrics to improve the quality of text descriptions. We further integrate the training of our model with maximum likelihood estimation (MLE), attribute embedding, and Reinforcement Learning (RL). To facilitate the learning, we build a new FAshion CAptioning Dataset (FACAD), which contains 993K images and 130K corresponding enchanting and diverse descriptions. Experiments on FACAD demonstrate the effectiveness of our model.

==> fc.tex <==
\section{Respecting Semantics for Fashion Captioning}
In this section, we briefly introduce encoder-decoder architecture with attention mechanism to solve the fashion captioning problem.

Our model takes a single image $\mathbf{x}$ and generates a caption $\mathbf{y}=\{ y_1,\ldots ,y_T \}$, with $y_i \in V^K$, $V^K$ is the vocabulary of $K$ words, $T$ is the caption length.
The objective of our model is to minimize the negative log-likelihood of the correct caption:
\begin{equation}
    \mathcal{L}=-\sum_{(\mathbf{x}, \mathbf{y})}\log p(\mathbf{y}\vert \mathbf{x})
\label{eq:loglikelihood}.
\end{equation}
To make sure that the caption correctly describe image attributes, we introduce an attribute feature $\mathbf{z}$ into the model. The objective then becomes:
\begin{equation}
    \mathcal{L}=-\sum_{(\mathbf{x}, \mathbf{y})}\log p(\mathbf{y}\vert \mathbf{x})=-\sum_{(\mathbf{x}, \mathbf{y})}\log p(\mathbf{y}\vert \mathbf{z}, \mathbf{x})p(\mathbf{z}\vert \mathbf{x})
\label{eq:loglikelihood_z}.
\end{equation}
Using chain rule, the objective can be decomposed over a sequence of words:
\begin{equation}
    \mathcal{L} = -\sum_{t=1}^{T}\log p(y_t\vert y_{1:t-1}, \mathbf{z}, \mathbf{x})
\end{equation}

We use encoder-decoder with attention mechanism to model this objective. The encoder is a convolutional neural network, which takes an image as the input and extract an image feature $\mathbf{x}$. We then input it into a decoder which is a Long Short-Term Memory (LSTM) network to capture the long-term consistency of the generated caption. The decoder predicts one word at a time and controls the fluency of the generated sentence. More specifically, we predicting the word at the $t$-th step, the decoder taks as input the feature of the image $\mathbf{x}$, the word embedding of the previous generated word $\mathbf{q}_{t-1}$ and the previous hidden state $\mathbf{h}_{t-1}$. The decoder then outputs a hidden state $\mathbf{h}_{t}$ and applies a linear layer $f$ to get the probability of choosing the next word:
\begin{equation}
    \mathbf{h}_{t} = LSTM([\mathbf{q}_{t-1};\mathbf{x}], \mathbf{h}_{t-1})
    \label{eq:hid}
\end{equation}
\begin{equation}
    p_{\theta}(y_t\vert y_{1:t-1}, \mathbf{x})=softmax(f(\mathbf{h}_{t}))
    \label{eq:y}
\end{equation}

\subsection{Visual Attribute Predictor}
Using the attribute vocabulary built in Section~\ref{sec:data}, we can associate each image with a set of attributes according to its captions. We then wish to precit the attributes given a test image. We treat this as a multi-label classification problem.

Fig.~\ref{fig:model} summarizes the attribute prediction network. It shares a CNN backbone with image feature extractor of captioning model. Then a linear layer is attached to the backbone. The output of the last linear layer is fed into a $c$-way softmax, where $c$ is the attribute vocabulary size. 
For a given training sample, let $\mathbf{l}_i=[ l_i^1,\ldots , l_i^c ]$ be the label vector of it, where $l_i^j=1$ if the image is annotated with $j$-th attribute, and $l_i^j=0$ otherwise. Let $\mathbf{a}_i=[ a_i^1,\ldots ,a_i^c ]$ be the predictive probability vector. Then the element-wise logistic loss function of the attribute predictor can be defined as:
\begin{equation}
    \mathcal{L}_{a}=\sum_{j=1}^c\log (1+exp(-l_i^ja_i^j))
\end{equation}

\subsection{Fashion Captioning with Attribute Embedding}
Combining all above, we can modify eq.~\ref{eq:hid} and eq.~\ref{eq:y} to include attribute features by:
\begin{equation}
    \mathbf{h}_{t} = LSTM([\mathbf{q}_{t-1};\mathbf{x};\mathbf{z}], \mathbf{h}_{t-1})
    \label{eq:hid}
\end{equation}
\begin{equation}
    p_{\theta}(y_t\vert y_{1:t-1}, \mathbf{x}, \mathbf{z})=softmax(f(\mathbf{h}_{t}))
    \label{eq:y}
\end{equation}
where $[\mathbf{q}_{t-1};\mathbf{x};\mathbf{z}]$ means that we simply concatenate those features together.

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{model.png}
\caption{The proposed model architecture and rewards.}
\label{fig:model}
\vspace{-0.15in}
\end{figure}


